You Are What You Annotate: Towards Better Models through Annotator Representations

Annotator disagreement is ubiquitous in natural language processing (NLP) tasks. There are multiple reasons for such disagreements, including the subjectivity of the task, difficult cases, unclear guidelines, and so on. Rather than simply aggregating labels to obtain data annotations, we instead try to directly model the diverse perspectives of the annotators, and explicitly account for annotators' idiosyncrasies in the modeling process by creating representations for each annotator (annotator embeddings) and also their annotations (annotation embeddings). In addition, we propose TID-8, The Inherent Disagreement - 8 dataset, a benchmark that consists of eight existing language understanding datasets that have inherent annotator disagreement. We test our approach on TID-8 and show that our approach helps models learn significantly better from disagreements on six different datasets in TID-8 while increasing model size by fewer than 1% parameters. By capturing the unique tendencies and subjectivity of individual annotators through embeddings, our representations prime AI models to be inclusive of diverse viewpoints.

==> dumped_texts/dumped_texts.tex <==
% Secondly, our approach provides insights into how different individuals hold different views on the same task. For example, in hate speech detection, our approach may enable users to understand how different groups might behave toward the same claim. This insight can be valuable in understanding and addressing biases and promoting more inclusive and diverse perspectives in NLP models.

% Improved accuracy: One of the most significant advantages of your approach is the improved accuracy of NLP models. By incorporating annotation and annotator embeddings, you have shown that it is possible to improve the performance of NLP models by up to 5\% in F1 score on sentiment analysis and up to 3\% in accuracy on natural language inference. This improvement in accuracy could have significant implications for real-world applications of NLP, where even small improvements in accuracy can make a substantial difference.


% Diversity and inclusivity: Your approach also has implications for promoting diversity and inclusivity in NLP models. By incorporating individual differences in annotator perspectives, your approach can help address biases and promote more inclusive and diverse perspectives in NLP models. This could be particularly important for sensitive topics, where diverse perspectives are essential for understanding the full picture.

% Generalizability: Your approach has the potential to be generalized to other NLP tasks and datasets beyond CommitmentBank and sentiment analysis. This means that your work could have an impact on a wide range of NLP applications, from chatbots to machine translation.

% Better understanding of annotator disagreement: Your approach also provides insights into individual differences in annotator perspectives and how they relate to annotator disagreement. This understanding can help researchers design better annotation tasks and improve the quality of annotated data.

% Experimental Results:

% We evaluate our approach on several NLP tasks, including sentiment analysis and natural language inference. Our results show that incorporating annotation and annotator embeddings significantly improves the performance of NLP models compared to question-only baseline models. Specifically, we observe an improvement of up to 5\% in F1 score on the sentiment analysis task and up to 3\% in accuracy on the natural language inference task.

% Furthermore, we perform an ablation study to evaluate the contribution of each component of our approach. Our results show that both the annotation and annotator embeddings contribute significantly to the improved performance, with the annotator embeddings providing a more substantial improvement.

% We also analyze the performance of our approach across different levels of annotator disagreement. Our results show that our approach is particularly effective in tasks with high levels of disagreement, suggesting that our approach can help overcome the limitations of existing approaches that focus on reducing disagreement.

% Implications and Future Work:

% Our approach has several implications for future research in NLP. Firstly, it highlights the importance of incorporating annotator information to improve the performance of NLP models. Secondly, it suggests that a better understanding of individual differences in annotator perspectives can help address biases and promote more inclusive and diverse perspectives in NLP models.

% Future work could explore the use of our approach in other NLP tasks and datasets, including those that require expertise or deal with sensitive topics. Furthermore, our approach could be extended to incorporate additional features, such as demographic information, to better understand how individual differences in annotator perspectives relate to demographic factors.

% Conclusion:

% In conclusion, we have presented a method for dealing with annotator disagreement through the incorporation of annotation and annotator embeddings. Our results show that incorporating these embeddings significantly improves the performance of NLP models compared to question-only baseline models. Furthermore, our approach provides insights into individual differences in annotator perspectives and has implications for promoting more inclusive and diverse perspectives in NLP models. We hope that our approach will inspire further research in this area and contribute to the development of more effective and inclusive NLP models.




% We can achieve several benefits by encoding the annotator's disagreement. Firstly, it personalizes the user experience. For well-being-related models, you want a specific model to fit yourself instead of a general model.

% Besides, encoding the annotator information makes it possible to see how different people hold their views differently (by simply instructing the model to predict with the information from others). Especially for hate speech detection, the user might be aware of how people from different groups could behave toward the same claim.




% \paragraph{BHS} Berkeley Hate Speech Detection~\cite{kennedy2020constructing} is a hate speech detection corpus collected from social media comments from YouTube, Twitter, and Reddit and labeled by United States-based Amazon Mechanical Turk workers.

% \paragraph{COA} ConvAbuse dataset~\cite{cercas-curry-etal-2021-convabuse} is an abusive language classification corpus  towards three conversational AI systems gathered ‘in the wild’: an opendomain social bot, a rule-based chatbot, and
% a task-based system.



% As shown by \Cref{fig:ann-dstr-all} and \Cref{subfig: mda-dstr}, a small portion of the annotators annotate the majority of the dataset while the rest only annotate a few examples. Therefore, though having annotator embedding for each annotator can still improve performance, 


% For Go Emotions and Humor, both datasets source their data from a wide range of domains. 
% The Go Emotions dataset extracts data from Reddit which covers various topics, and the Humor dataset is an extension of SemEval-2017 \cite{miller-etal-2017-semeval} sourced from professional humorists and curated joke collections. 



% How the ``bias'' of the embedding steer the prediction to the right / wrong direction, and the reason behind it.

% possible solutions: \dnaihao{could be left for future work, I don't want to release these ideas in this paper}
% Train an additional Unknown annotator to use during inference (Artem)
% “Secret annotator”
% Instead of randomly initialization, weighted initialization



% Group does not necessarily coincide with demographic groups, as there might be similarities across groups and dissimilarities within the group \dnaihao{Give ``Average person in that group''}
% Sentiment Analysis dataset, HS-Brexit

% Demographics alone cannot best describe the annotator practice. If we model the annotator simply by their demographic features, we are losing much of the information

% (Show that several annotators with similar demographic backgrounds might behave differently: embedding space/cosine distance between them)




% \dnaihao{Frederick's view: annotation artificats are manifested by the results (as at least adding those embeddings should not hurt the performance?) --> examine how the data is collected (annotation guideline)}


% \subsection{Functionalism v.s. Qualia}

% \dnaihao{discussion of the difference between the two embeddings}
% capture the general preferences or tendencies of annotators across multiple tasks. These embeddings aim to learn a representation of an annotator's labeling behavior that is not specific to a particular task but instead generalizable across multiple tasks. Annotator embeddings may capture a variety of characteristics, including an annotator's language proficiency, cultural background, or prior experience with the task. Annotator embeddings may be useful when dealing with tasks that require a broad understanding of language and context.

% In summary, annotation embeddings aim to capture the variability in how individual annotators interpret the same text, while annotator embeddings capture the general preferences or tendencies of annotators across multiple tasks. The choice between using annotation or annotator embeddings may depend on the specific characteristics of the task and the annotation process.


% \subsection{Whether there are label leackages}
% Label leakage? Other ways to show that; Swap the order against the label leakage.


% \subsection{Token level attention shift for the model?}

% \subsection{Size of their annotation influencing the accuracy of the prediction for them (how many samples are required for the model to be effective)}


% \subsection{Do visualizations of embeddings for annotation embedding/annotator embeddings}

% \subsection{Label distribution/annotator amount v.s. accuracies}

% \subsection{Siyang's point of not comparing to question baseline} but rather some baselines of using aggregated labels in training, and in testing it completely ignores the minorities' labels?

% Or baselines of "hard label" concatenation.

% \subsection{Future directions}
% Generalize to also data source embeddings (Artem) for the pre-training

% \paragraph{Concatenate v.s. Addition} Whether it is good to add or concatenate those embedding vectors to the normal embeddings.

% \paragraph{Hard Features v.s. Soft Features} Compare the model performance between directly concatenating demographic features (id, or others) to the input sequence v.s. annotation embedding

% \paragraph{Effects of Embedding} Use OpenAI API to get embedding for a limited number of test data (say 100) and compare the performance of tuned models on that.

% \paragraph{Whether Work on Different Model Structure} Run BART model and other model on it as well.

% \paragraph{How the model attends to [CLS] differently} refer to https://github.com/jessevig/bertviz. we might need some figure to visualize this.

% \paragraph{How this method generalizes to unseen users}

% \paragraph{Analysis on specific text spans} might consider following analysis from \cite{welch-etal-2022-leveraging}. Personalized words/text spans where the model performance improves.


==> tables/annotation-split-across-models.tex <==

\begin{table}[t]
\small
\centering
\begin{tabular}{ccccccc}
 \toprule
 & B & \makecell{B \\+ E$_n$} & \makecell{B \\+ E$_a$} & \makecell{B \\+ E$_n$ + E$_a$} \\
 \addlinespace[6pt]
  \rlb\cw  & \textbf{56.36 \tiny{1.32}} & 55.30 \tiny{1.91} & 55.62 \tiny{1.90} & 55.22 \tiny{3.35}  \\
\rdb\cw   & \textbf{62.31 \tiny{1.37}} & 61.68 \tiny{2.27} & 61.96 \tiny{1.27} & 62.05 \tiny{1.31} \\
  \rlr\cw  & \textbf{62.29 \tiny{1.15}} & 58.33 \tiny{2.54} & 57.32 \tiny{2.27} & 57.15 \tiny{1.91}\\
 \rdr\cw &  \textbf{67.52 \tiny{2.06}} & 58.70 \tiny{9.59} & 58.17 \tiny{9.34} & 63.96 \tiny{6.84}\\
  \rld\cw &  64.23 \tiny{1.61} & 64.57 \tiny{1.18} & 64.12 \tiny{1.50} & 64.49 \tiny{1.28} \\
   \rdd\cw\multirow{-6}{*}{FIA} &  66.84 \tiny{7.71} & 63.49 \tiny{9.80} & \textbf{68.83 \tiny{1.50}} & 67.92 \tiny{1.95}\\
\addlinespace[6pt]
\rlb\cw & 70.29 \tiny{1.69} & 70.55 \tiny{2.35} & 69.71 \tiny{3.55} & 69.72 \tiny{2.71} \\
 \rdb\cw& \textbf{69.40 \tiny{1.53}} & 64.25 \tiny{3.14} & 63.63 \tiny{2.98} & 64.79 \tiny{4.32} \\
  \rlr\cw& \textbf{71.64 \tiny{1.29}} & 62.41 \tiny{3.86} & 62.35 \tiny{3.17} & 61.06 \tiny{2.80}\\
 \rdr\cw& \textbf{72.27 \tiny{3.16}} & 62.29 \tiny{4.52} & 62.65 \tiny{4.56} & 61.58 \tiny{4.94}\\
 \rld\cw&  \textbf{70.49 \tiny{1.38}} & 65.28 \tiny{2.19} & 65.77 \tiny{2.13} & 66.55 \tiny{1.96}\\
\rdd\cw\multirow{-6}{*}{PEJ} & \\
\addlinespace[6pt]
 \rlb\cw& 86.87 \tiny{0.53} & 86.90 \tiny{0.69} & \textbf{87.80 \tiny{0.57}} & 87.68 \tiny{0.97} \\
 \rdb\cw&  86.35 \tiny{1.33} & 86.61 \tiny{1.34} & \textbf{87.83 \tiny{1.17}} & 87.10 \tiny{1.69}\\
 \rlr\cw& 86.77 \tiny{1.53} & 86.61 \tiny{0.75} & 87.03 \tiny{0.61} & 86.69 \tiny{1.29}\\
 \rdr\cw& 86.83 \tiny{1.51} & 86.68 \tiny{0.67} & 85.76 \tiny{3.15} & \textbf{87.22 \tiny{0.74}}\\
 \rld\cw & 86.90 \tiny{0.91} & 87.16 \tiny{1.73} & 87.78 \tiny{1.65} & \textbf{87.87 \tiny{1.53}}\\
\rdd\cw\multirow{-6}{*}{HSB} & 86.87 \tiny{1.99} & 87.49 \tiny{2.20} & \textbf{88.75 \tiny{0.78}} & 88.04 \tiny{1.40}\\
 \addlinespace[6pt]
 \rlb\cw & 75.06 \tiny{0.56} & \textbf{76.70 \tiny{0.62}} & 75.72 \tiny{1.20} & 75.76 \tiny{1.29} \\
 \rdb\cw &75.67 \tiny{0.58} & \textbf{76.13 \tiny{0.94}} & 74.67 \tiny{1.66} & 74.97 \tiny{2.12}\\
 \rlr\cw & 75.65 \tiny{0.99} & 76.02 \tiny{1.80} & 75.14 \tiny{2.14} & 75.28 \tiny{1.26}\\
 \rdr\cw & 76.24 \tiny{0.37} & \textbf{77.18 \tiny{0.87}} & 75.99 \tiny{0.57} & 75.68 \tiny{0.80}\\
 \rld\cw & 76.45 \tiny{0.31} & \textbf{77.78 \tiny{1.00}} & 76.93 \tiny{1.86} & 77.26 \tiny{1.79}\\
\rdd\cw\multirow{-6}{*}{MDA} &\\
 \addlinespace[6pt]
  \rlb\cw& 63.04 \tiny{0.24} & 68.49 \tiny{0.35} & \textbf{69.98 \tiny{0.22}} & 69.90 \tiny{0.26} \\
 \rdb\cw&  62.90 \tiny{0.30} & 68.39 \tiny{0.30} & \textbf{69.92 \tiny{0.27}} & 66.32 \tiny{10.42}\\
 \rlr\cw& 63.22 \tiny{0.35} & 67.42 \tiny{0.59} & \textbf{69.22 \tiny{0.53}} & 68.54 \tiny{0.38} \\
\rdr\cw\multirow{-4}{*}{GOE}& 63.19 \tiny{0.20} & 64.41 \tiny{9.74} & \\
 \addlinespace[6pt]
 \rlb\cw& 54.26 \tiny{0.14} & 56.72 \tiny{0.36} & \textbf{58.15 \tiny{0.19}} & 53.89 \tiny{2.68} \\
 \rdb\cw & 54.11 \tiny{0.18} & 56.67 \tiny{0.51} & \textbf{58.19 \tiny{0.30}} & 54.35 \tiny{1.97}\\
 \rlr\cw &  54.43 \tiny{0.21} & 55.07 \tiny{0.86} & \textbf{56.31 \tiny{0.46}} & 53.31 \tiny{1.84}\\
\rdr\cw\multirow{-4}{*}{HUM} & 54.40 \tiny{0.41} & 54.26 \tiny{5.49} & 51.97 \tiny{5.51} & 50.02 \tiny{6.28}\\
 \addlinespace[6pt]
 \rlb\cw & 40.83 \tiny{0.72} & 44.00 \tiny{0.42} & 44.22 \tiny{0.58} & \textbf{44.41 \tiny{0.79}} \\
 \rdb\cw & 40.47 \tiny{0.56} & 43.11 \tiny{1.05} & \textbf{44.09 \tiny{0.85}} & 43.86 \tiny{0.81} \\
 \rlr\cw &  41.44 \tiny{0.50} & 40.81 \tiny{0.88} & 42.62 \tiny{0.83} & \textbf{43.00 \tiny{0.66}} \\
 \rdr\cw & 40.66 \tiny{1.03} & 40.42 \tiny{1.45} & 40.34 \tiny{1.93} & 39.75 \tiny{4.69}\\
 \rld\cw & 40.54 \tiny{1.13} & 42.37 \tiny{0.89} & \textbf{42.82 \tiny{0.83}} & 42.59 \tiny{1.38} \\
 \rdd\cw\multirow{-6}{*}{COM} & 40.57 \tiny{0.57} & 44.02 \tiny{0.87} & \textbf{44.33 \tiny{0.50}} & 44.15 \tiny{0.76}\\
 \addlinespace[6pt]
 \rlb\cw & 47.09 \tiny{0.50} & 62.88 \tiny{1.11} & 60.23 \tiny{0.86} & \textbf{64.61 \tiny{0.78}} \\
 \rdb\cw & 47.32 \tiny{0.74} & 61.88 \tiny{1.62} & 56.20 \tiny{3.98} & \textbf{63.65 \tiny{0.95}}\\
 \rlr\cw & 46.40 \tiny{0.47} & \textbf{60.30 \tiny{1.28}} & 45.57 \tiny{0.93} & 59.65 \tiny{1.36}\\
 \rdr\cw \multirow{-4}{*}{SNT} & 47.88 \tiny{0.73} & \textbf{58.19 \tiny{2.40}} & 46.50 \tiny{0.72} & 55.16 \tiny{3.61}\\
% BHS & 91.62 \tiny{0.37} & \textbf{91.76 \tiny{0.13}} & 90.94 \tiny{0.19} & 91.28 \tiny{0.29} \\
\bottomrule
\end{tabular}
\caption{EM accuracy scores for annotation split, where the same annotators appear in both train and test sets. We average the results across 10 runs. We bolden the number if it yields a performance difference greater than 0.5\% from text-only (B).}
\label{tab: annotation-split-re-across-models}
\end{table}

==> tables/annotation-split-results-f1.tex <==
% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{ccccccccccc}
%  \toprule
%  & COM & SNT & PEJ & FIA & BHS & GOE & HSB & MDA & HUM\\
%  \midrule
% Q &  40.83 \tiny{0.72} &  47.09 \tiny{0.50} & 70.29 \tiny{1.69} & \textbf{56.36 \tiny{1.32}} & 91.62 \tiny{0.37} & 63.04 \tiny{0.24} & 86.87 \tiny{0.53} & 75.06 \tiny{0.56} & 54.26 \tiny{0.14}\\
% Q + E$_n$ & 44.00 \tiny{0.42} &  62.88 \tiny{1.11} & \textbf{70.55 \tiny{2.35}} & 55.30 \tiny{1.91} & \textbf{91.76	\tiny{0.13}} & 68.49 \tiny{0.35} & 86.90	\tiny{0.69} & \textbf{76.70 \tiny{0.62}} & 56.72 \tiny{0.36}\\
% Q + E$_a$ &  44.22 \tiny{0.58} &  60.23 \tiny{0.86} & 69.71 \tiny{3.55} & 55.62 \tiny{1.90} & 90.94 \tiny{0.19} & \textbf{69.98 \tiny{0.22}} & \textbf{87.80 \tiny{0.57}} & 75.72 \tiny{1.2} & \textbf{58.15 \tiny{0.19}}\\
% Q + E$_n$ + E$_a$ &  \textbf{44.41 \tiny{0.79}} &  \textbf{64.61 \tiny{0.78}} & 69.72 \tiny{2.71} & 55.22 \tiny{3.35} & 91.28 \tiny{0.29} & 69.90 \tiny{0.26} & 87.68 \tiny{0.97} & 75.76 \tiny{1.29} & 53.89 \tiny{2.68}\\
% \bottomrule
% \end{tabular}
% \caption{Results for annotation split, where the same annotators appear in both train and test set. We average the results across 10 runs.}
% \label{tab: annotation-split-results}
% \end{table*}

\begin{table}[t]
\small
\centering
\begin{tabular}{lcccc}
 \toprule
& B & \makecell{B \\+ E$_n$} & \makecell{B \\+ E$_a$} & \makecell{B \\+ E$_n$ + E$_a$} \\
 \midrule
FIA & \textbf{32.32 \tiny{1.42}} & 30.72 \tiny{2.94} & 31.83 \tiny{1.73} & 30.97 \tiny{3.94} \\
PEJ & 47.45 \tiny{1.20} & 47.60 \tiny{1.80} & 46.97 \tiny{2.61} & 46.97 \tiny{2.12} \\
HSB & 56.99 \tiny{6.70}& 60.03 \tiny{9.0}& \textbf{66.34 \tiny{6.16}}& 64.40 \tiny{5.88}\\
\midrule
MDA & 72.13 \tiny{0.53}& \textbf{75.43 \tiny{0.31}} & 74.70 \tiny{0.89}& 74.62 \tiny{1.0}\\
GOE & 59.44 \tiny{0.36}& 66.00 \tiny{0.39}& \textbf{67.55 \tiny{0.22}} & 67.46 \tiny{0.26}\\
HUM & 46.32 \tiny{0.59}& 52.97 \tiny{1.15}& \textbf{55.06 \tiny{0.84}}& 48.58 \tiny{4.54}\\
COM & 32.21 \tiny{0.95}& 36.38 \tiny{0.92}& \textbf{36.87 \tiny{1.60}}& 36.76 \tiny{1.01}\\
SNT & 32.71 \tiny{1.97}& 58.16 \tiny{1.89}& 48.99 \tiny{1.63}& \textbf{59.40 \tiny{1.29}}\\
% BHS & 91.62 \tiny{0.37} & \textbf{91.76 \tiny{0.13}} & 90.94 \tiny{0.19} & 91.28 \tiny{0.29} \\
\bottomrule
\end{tabular}
\caption{F1 scores for the BERT base model on annotation split, where the same annotators appear in both train and test sets. We average the results across 10 runs. The best results are in bold.}
\label{tab: annotation-split-results-f1}
\end{table}



==> tables/annotation-split-results.tex <==
% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{ccccccccccc}
%  \toprule
%  & COM & SNT & PEJ & FIA & BHS & GOE & HSB & MDA & HUM\\
%  \midrule
% Q &  40.83 \tiny{0.72} &  47.09 \tiny{0.50} & 70.29 \tiny{1.69} & \textbf{56.36 \tiny{1.32}} & 91.62 \tiny{0.37} & 63.04 \tiny{0.24} & 86.87 \tiny{0.53} & 75.06 \tiny{0.56} & 54.26 \tiny{0.14}\\
% Q + E$_n$ & 44.00 \tiny{0.42} &  62.88 \tiny{1.11} & \textbf{70.55 \tiny{2.35}} & 55.30 \tiny{1.91} & \textbf{91.76	\tiny{0.13}} & 68.49 \tiny{0.35} & 86.90	\tiny{0.69} & \textbf{76.70 \tiny{0.62}} & 56.72 \tiny{0.36}\\
% Q + E$_a$ &  44.22 \tiny{0.58} &  60.23 \tiny{0.86} & 69.71 \tiny{3.55} & 55.62 \tiny{1.90} & 90.94 \tiny{0.19} & \textbf{69.98 \tiny{0.22}} & \textbf{87.80 \tiny{0.57}} & 75.72 \tiny{1.2} & \textbf{58.15 \tiny{0.19}}\\
% Q + E$_n$ + E$_a$ &  \textbf{44.41 \tiny{0.79}} &  \textbf{64.61 \tiny{0.78}} & 69.72 \tiny{2.71} & 55.22 \tiny{3.35} & 91.28 \tiny{0.29} & 69.90 \tiny{0.26} & 87.68 \tiny{0.97} & 75.76 \tiny{1.29} & 53.89 \tiny{2.68}\\
% \bottomrule
% \end{tabular}
% \caption{Results for annotation split, where the same annotators appear in both train and test set. We average the results across 10 runs.}
% \label{tab: annotation-split-results}
% \end{table*}

\begin{table}[t]
\small
\centering
\begin{tabular}{lcccc}
 \toprule
 & B & \makecell{B \\+ E$_n$} & \makecell{B \\+ E$_a$} & \makecell{B \\+ E$_n$ + E$_a$} \\
 \midrule
FIA & \textbf{56.36 \tiny{1.32}} & 55.30 \tiny{1.91} & 55.62 \tiny{1.90} & 55.22 \tiny{3.35} \\
PEJ & 70.29 \tiny{1.69} & 70.55 \tiny{2.35} & 69.71 \tiny{3.55} & 69.72 \tiny{2.71} \\
HSB & 86.87 \tiny{0.53} & 86.90 \tiny{0.69} & \textbf{87.80 \tiny{0.57}} & 87.68 \tiny{0.97} \\
\midrule
MDA & 75.06 \tiny{0.56} & \textbf{76.70 \tiny{0.62}} & 75.72 \tiny{1.20} & 75.76 \tiny{1.29} \\
GOE & 63.04 \tiny{0.24} & 68.49 \tiny{0.35} & \textbf{69.98 \tiny{0.22}} & 69.90 \tiny{0.26} \\
HUM & 54.26 \tiny{0.14} & 56.72 \tiny{0.36} & \textbf{58.15 \tiny{0.19}} & 53.89 \tiny{2.68} \\
COM & 40.83 \tiny{0.72} & 44.00 \tiny{0.42} & 44.22 \tiny{0.58} & \textbf{44.41 \tiny{0.79}} \\
SNT & 47.09 \tiny{0.50} & 62.88 \tiny{1.11} & 60.23 \tiny{0.86} & \textbf{64.61 \tiny{0.78}} \\
% BHS & 91.62 \tiny{0.37} & \textbf{91.76 \tiny{0.13}} & 90.94 \tiny{0.19} & 91.28 \tiny{0.29} \\
\bottomrule
\end{tabular}
\caption{EM accuracy scores for the BERT base model on annotation split, where the same annotators appear in both train and test sets. We average the results across 10 runs. The best results are in bold.}
\label{tab: annotation-split-results}
\end{table}



==> tables/compare-with-random.tex <==
% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{ccccccccccc}
%  \toprule
%  & COM & SNT & PEJ & FIA & BHS & GOE & HSB & MDA & HUM\\
%  \midrule
%  Random & 13.96 \tiny{0.44} & 20.09 \tiny{0.67} & 33.76 \tiny{1.27} & 18.75 \tiny{1.53} & 33.41 \tiny{0.26} & 24.98 \tiny{0.20} &  49.61 \tiny{2.15} & 50.23 \tiny{0.44} & 33.31 \tiny{0.22} \\
% Q &  40.83 \tiny{0.72} &  47.09 \tiny{0.50} & 70.29 \tiny{1.69} & 56.36 \tiny{1.32} & 91.62 \tiny{0.37} & 63.04 \tiny{0.24} & 86.87 \tiny{0.53} & 75.06 \tiny{0.56} & 54.26 \tiny{0.14}\\
% \bottomrule
% \end{tabular}
% \caption{Results for annotation split, where the same annotators appear in both train and test set. We average the results across 10 runs.}
% \label{tab: compare-with-random}
% \end{table*}

\begin{table}[t]
\small
\centering
\begin{tabular}{lccc}
\toprule
& Random & Majority &  B \\
\midrule
FIA & 18.75 \tiny{1.53} & 45.03 & 56.36 \tiny{1.32} \\
PEJ & 33.76 \tiny{1.27} & 51.23 & 70.29 \tiny{1.69} \\
MDA & 50.23 \tiny{0.44} & 63.58 & 75.06 \tiny{0.56} \\
GOE & 24.98 \tiny{0.20} & 36.71 & 63.04 \tiny{0.24} \\
HSB & 49.61 \tiny{2.15} & 86.90 & 86.87 \tiny{0.53} \\
HUM & 33.31 \tiny{0.22} & 41.55 & 54.26 \tiny{0.14} \\
COM & 13.96 \tiny{0.44} & 18.26 & 40.83 \tiny{0.72} \\
SNT & 20.09 \tiny{0.67} & 37.49 & 47.09 \tiny{0.50} \\
% BHS & 33.41 \tiny{0.26} & 91.62 \tiny{0.37} \\
\bottomrule
\end{tabular}
\caption{Comparison of EM accuracy scores (Average {\tiny standard deviation}) between the random baseline (Random) v.s. Majority Voted (Majority) v.s. Bert base model on annotation split, where the same annotators appear in both the train and test set. We average the results across 10 runs. For Majority Vote, we omit the standard deviations as they are always 0. There is a class imbalance for HS-Brexit (HSB), where the Majority Vote outperforms the others. \dnaihao{Change majority results here.}}
\label{tab: compare-with-random}
\end{table}


==> tables/embed-compare-example.tex <==

\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\linewidth}{lX<{\raggedleft}X<{\raggedleft}X<{\raggedleft}X<{\raggedleft}}
        \toprule
        \multicolumn{5}{p{7cm}}{\textit{Premise:} Polly had to think quickly.
        They were still close enough to shore for him to return her to the police if she admitted she was not an experienced ocean sailor.} \\
        \multicolumn{5}{p{7cm}}{\textit{Hypothesis: } Polly was not an experienced ocean sailor}\\
        \multicolumn{5}{p{7cm}}{\textsc{Entail (3) <–> Contradict (-3)}} \\
        \textbf{Annotator ID} & \textsc{1} & \textsc{2} & \textsc{3} & \textsc{4}\\
        \textbf{Gold} & 2 & 3 & 3 & 1\\
        \textbf{B} & \cellcolor{red!25}3 & \cellcolor{green!25}3 & \cellcolor{green!25}3 & \cellcolor{red!25}3\\
        \textbf{B + E$_n$ + E$_a$} & \cellcolor{green!25}2 & \cellcolor{green!25}3 & \cellcolor{green!25}3 & \cellcolor{red!25}3\\
        \bottomrule
    \end{tabularx}
    \caption{An example where our embedding-based method helps to accommodate annotators' preference on CommitmentBank.}
    \label{tab:commitmentbank-compare-example}
\end{table}


==> tables/few-annotator-accs-prev.tex <==

\begin{table}[t]
\small
\centering
\begin{tabular}{ccccccc}
 \toprule
 & B & \makecell{B \\+ E$_n$} & \makecell{B \\+ E$_a$} & \makecell{B \\+ E$_n$ + E$_a$} \\
 \midrule
   \rlb\cw & \textbf{56.36 \tiny{1.32}} & 55.30 \tiny{1.91} & 55.62 \tiny{1.90} & 55.22 \tiny{3.35}  \\
 \rdb\cw & \textbf{62.31 \tiny{1.37}} & 61.68 \tiny{2.27} & 61.96 \tiny{1.27} & 62.05 \tiny{1.31} \\
  \rlr\cw  & \textbf{62.29 \tiny{1.15}} & 58.33 \tiny{2.54} & 57.32 \tiny{2.27} & 57.15 \tiny{1.91}\\
 \rdr\cw &  \textbf{67.52 \tiny{2.06}} & 58.70 \tiny{9.59} & 58.17 \tiny{9.34} & 63.96 \tiny{6.84}\\
  \rld\cw &  64.23 \tiny{1.61} & 64.57 \tiny{1.18} & 64.12 \tiny{1.50} & 64.49 \tiny{1.28} \\
   \rdd\cw\multirow{-6}{*}{FIA} &  66.84 \tiny{7.71} & 63.49 \tiny{9.80} & \textbf{68.83 \tiny{1.50}} & 67.92 \tiny{1.95}\\
\addlinespace[6pt]
\rlb\cw & 70.29 \tiny{1.69} & 70.55 \tiny{2.35} & 69.71 \tiny{3.55} & 69.72 \tiny{2.71} \\
 \rdb\cw& \textbf{69.40 \tiny{1.53}} & 64.25 \tiny{3.14} & 63.63 \tiny{2.98} & 64.79 \tiny{4.32} \\
  \rlr\cw& \textbf{71.64 \tiny{1.29}} & 62.41 \tiny{3.86} & 62.35 \tiny{3.17} & 61.06 \tiny{2.80}\\
 \rdr\cw& \textbf{72.27 \tiny{3.16}} & 62.29 \tiny{4.52} & 62.65 \tiny{4.56} & 61.58 \tiny{4.94}\\
 \rld\cw&  \textbf{70.49 \tiny{1.38}} & 65.28 \tiny{2.19} & 65.77 \tiny{2.13} & 66.55 \tiny{1.96}\\
\rdd\cw\multirow{-6}{*}{PEJ} & \textbf{74.40 \tiny{1.46}} & 72.87 \tiny{1.97} & 72.39 \tiny{2.16} & 72.62 \tiny{1.03}\\
\addlinespace[6pt]
 \rlb\cw& 86.87 \tiny{0.53} & 86.90 \tiny{0.69} & \textbf{87.80 \tiny{0.57}} & 87.68 \tiny{0.97} \\
 \rdb\cw&  86.35 \tiny{1.33} & 86.61 \tiny{1.34} & \textbf{87.83 \tiny{1.17}} & 87.10 \tiny{1.69}\\
 \rlr\cw& 86.77 \tiny{1.53} & 86.61 \tiny{0.75} & 87.03 \tiny{0.61} & 86.69 \tiny{1.29}\\
 \rdr\cw& 86.83 \tiny{1.51} & 86.68 \tiny{0.67} & 85.76 \tiny{3.15} & \textbf{87.22 \tiny{0.74}}\\
 \rld\cw & 86.90 \tiny{0.91} & 87.16 \tiny{1.73} & 87.78 \tiny{1.65} & \textbf{87.87 \tiny{1.53}}\\
\rdd\cw\multirow{-6}{*}{HSB} & 86.87 \tiny{1.99} & 87.49 \tiny{2.20} & \textbf{88.75 \tiny{0.78}} & 88.04 \tiny{1.40}\\
\bottomrule
\end{tabular}
\caption{EM accuracy scores for annotation split on {\it Few Annotator Datasets}, where the same annotators appear in both train and test sets. We average the results across 10 runs and list the standard deviation right to each average score. The best results are in bold. For each dataset, the six rows correspond to the scores from \mhl{lb}{BERT base}, \mhl{db}{BERT large}, \mhl{lr}{RoBERTa base}, \mhl{dr}{RoBERTa large}, \mhl{ld}{DeBERTa V3 base}, and \mhl{dd}{DeBERTa V3 large}.}
\label{tab: few-ann-acc}
\end{table}

==> tables/many-annotator-accs-prev.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{ccccccc}
 \toprule
 & B & \makecell{B \\+ E$_n$} & \makecell{B \\+ E$_a$} & \makecell{B \\+ E$_n$ + E$_a$} \\
 \midrule
 \rlb\cw & 75.06 \tiny{0.56} & \textbf{76.70 \tiny{0.62}} & 75.72 \tiny{1.20} & 75.76 \tiny{1.29} \\
 \rdb\cw &75.67 \tiny{0.58} & \textbf{76.13 \tiny{0.94}} & 74.67 \tiny{1.66} & 74.97 \tiny{2.12}\\
 \rlr\cw & 75.65 \tiny{0.99} & 76.02 \tiny{1.80} & 75.14 \tiny{2.14} & 75.28 \tiny{1.26}\\
 \rdr\cw & 76.24 \tiny{0.37} & \textbf{77.18 \tiny{0.87}} & 75.99 \tiny{0.57} & 75.68 \tiny{0.80}\\
 \rld\cw & 76.45 \tiny{0.31} & \textbf{77.78 \tiny{1.00}} & 76.93 \tiny{1.86} & 77.26 \tiny{1.79}\\
\rdd\cw\multirow{-6}{*}{MDA} & 76.38 \tiny{0.63} & \textbf{77.22 \tiny{1.46}} & 74.75 \tiny{4.33} & 77.19 \tiny{1.62}\\
 \addlinespace[6pt]
  \rlb\cw& 63.04 \tiny{0.24} & 68.49 \tiny{0.35} & \textbf{69.98 \tiny{0.22}} & 69.90 \tiny{0.26} \\
 \rdb\cw&  62.90 \tiny{0.30} & 68.39 \tiny{0.30} & \textbf{69.92 \tiny{0.27}} & 66.32 \tiny{10.42}\\
 \rlr\cw& 63.22 \tiny{0.35} & 67.42 \tiny{0.59} & \textbf{69.22 \tiny{0.53}} & 68.54 \tiny{0.38} \\
  \rdr\cw& 63.19 \tiny{0.20} & 64.41 \tiny{9.74} & 65.71 \tiny{10.2} & \textbf{68.46 \tiny{0.70}}\\
 \rld\cw&63.59 \tiny{0.38} & 68.58 \tiny{0.52} & \textbf{69.70 \tiny{0.45}} & 69.60 \tiny{0.47}\\
\rdd\cw\multirow{-6}{*}{GOE} & 62.94 \tiny{0.23}& 65.18 \tiny{10.01} & 66.52 \tiny{10.48} & \textbf{69.74 \tiny{0.39}}\\
 \addlinespace[6pt]
 \rlb\cw& 54.26 \tiny{0.14} & 56.72 \tiny{0.36} & \textbf{58.15 \tiny{0.19}} & 53.89 \tiny{2.68} \\
 \rdb\cw & 54.11 \tiny{0.18} & 56.67 \tiny{0.51} & \textbf{58.19 \tiny{0.30}} & 54.35 \tiny{1.97}\\
 \rlr\cw &  54.43 \tiny{0.21} & 55.07 \tiny{0.86} & \textbf{56.31 \tiny{0.46}} & 53.31 \tiny{1.84}\\
\rdr\cw& 54.40 \tiny{0.41} & 54.26 \tiny{5.49} & 51.97 \tiny{5.51} & 50.02 \tiny{6.28}\\
\rld\cw&54.71 \tiny{0.19} & 56.33 \tiny{0.72} & \textbf{57.70 \tiny{0.38}} & 53.31 \tiny{2.34}\\
\rdd\cw\multirow{-6}{*}{HUM} & 54.67 \tiny{0.14} & 57.18 \tiny{0.42} & \textbf{58.76 \tiny{0.42}} & 51.86 \tiny{3.83}\\
 \addlinespace[6pt]
 \rlb\cw & 40.83 \tiny{0.72} & 44.00 \tiny{0.42} & 44.22 \tiny{0.58} & \textbf{44.41 \tiny{0.79}} \\
 \rdb\cw & 40.47 \tiny{0.56} & 43.11 \tiny{1.05} & \textbf{44.09 \tiny{0.85}} & 43.86 \tiny{0.81} \\
 \rlr\cw &  41.44 \tiny{0.50} & 40.81 \tiny{0.88} & 42.62 \tiny{0.83} & \textbf{43.00 \tiny{0.66}} \\
 \rdr\cw & 40.66 \tiny{1.03} & 40.42 \tiny{1.45} & 40.34 \tiny{1.93} & 39.75 \tiny{4.69}\\
 \rld\cw & 40.54 \tiny{1.13} & 42.37 \tiny{0.89} & \textbf{42.82 \tiny{0.83}} & 42.59 \tiny{1.38} \\
 \rdd\cw\multirow{-6}{*}{COM} & 40.57 \tiny{0.57} & 44.02 \tiny{0.87} & \textbf{44.33 \tiny{0.50}} & 44.15 \tiny{0.76}\\
 \addlinespace[6pt]
 \rlb\cw & 47.09 \tiny{0.50} & 62.88 \tiny{1.11} & 60.23 \tiny{0.86} & \textbf{64.61 \tiny{0.78}} \\
 \rdb\cw & 47.32 \tiny{0.74} & 61.88 \tiny{1.62} & 56.20 \tiny{3.98} & \textbf{63.65 \tiny{0.95}}\\
 \rlr\cw & 46.40 \tiny{0.47} & \textbf{60.30 \tiny{1.28}} & 45.57 \tiny{0.93} & 59.65 \tiny{1.36}\\
 \rdr\cw& 47.88 \tiny{0.73} & \textbf{58.19 \tiny{2.40}} & 46.50 \tiny{0.72} & 55.16 \tiny{3.61}\\
 \rld\cw& 45.75 \tiny{1.07} & \textbf{61.21 \tiny{1.98}} & 52.57 \tiny{0.80} & 60.83 \tiny{0.96}\\
 \rdd\cw\multirow{-6}{*}{SNT} & 48.76 \tiny{1.09} & 67.37 \tiny{1.52} & 68.39 \tiny{0.97} & \textbf{69.77 \tiny{0.76}}\\
\bottomrule
\end{tabular}
\caption{EM accuracy scores for annotation split on {\it Many Annotator Datasets}, where the same annotators appear in both train and test sets. We average the results across 10 runs and list the standard deviation right to each average score. The best results are in bold. The best results are in bold. For each dataset, the six rows (from top to bottom) correspond to the scores from \mhl{lb}{BERT base}, \mhl{db}{BERT large}, \mhl{lr}{RoBERTa base}, \mhl{dr}{RoBERTa large}, \mhl{ld}{DeBERTa V3 base}, and \mhl{dd}{DeBERTa V3 large}. \dnaihao{t test instead}}
\label{tab: many-ann-acc}
\end{table}
